Signal Convolution Logic

We introduce a new logic called Signal Convolution Logic (SCL) that combines temporal logic with convolutional filters from digital signal processing. SCL enables to reason about the percentage of time a formula is satisfied in a bounded interval. We demonstrate that this new logic is a suitable formalism to effectively express non-functional requirements in Cyber-Physical Systems displaying noisy and irregular behaviours. We define both a qualitative and quantitative semantics for it, providing an efficient monitoring procedure. Finally, we prove SCL at work to monitor the artificial pancreas controllers that are employed to automate the delivery of insulin for patients with type-1 diabetes.

==> monitoringold.tex <==
% !TEX root =  main.tex
\section{Monitoring Algorithm}
\label{sec:monitoring}
\todo{
Only the $<>$ algorithm is described in detail. Despite your claim that the "monitors for other kinds of formulas are standard", you say (earlier in that paragraph) that the algorithm for "AND" can access the queues. I would assume that the AND has to deal with the queues. //
Is the {\bf algorithm useful for recursive applications}, i.e., whenever a new signal value is coming in, the evaluator returns a valuation of the formula? Or does it need to process the data in batches.Algorithm in A: what is h?
}
We now provide two efficient monitor algorithms for the boolean 
semantics of SML formulas. The first method we present works 
for a subclass of kernels (mostly used in practice), 
satisfying a semigroup property.  The second method, 
instead, works for general kernels.

Consider an SML formula $\langle k_{[T_0,T_1]}, p \rangle \phi$ and a signal $\vec s$, we are interested in computing $\chi ( \vec s , t,\langle k_{[T_0,T_1]},  p \rangle \phi) =(g(t) - p \ge 0)$, as a function of $t$, where $g$ is the following convolution function
\begin{equation}
\label{eq:monitoring}
g(t) =  \int_{t+T_0}^{t+T_1} k_{[T_0,T_1]} (\tau-(t+T_0))  \chi(\vec s , \tau,\phi )  d\tau
\end{equation}

It follows that the efficient monitoring of the boolean semantics of SML is linked to the efficient evaluation of $g(t)-p$, which is possible if  $g(t+h)$ can be computed by reusing the value of $g(t)$ previously stored.
%The problem is related to the kernel of Equation \ref{eq:monitoring}, in fact calculating $f(t+h)$ means translating the windows interval from  ${[T_0,T_1]}$ to ${[T_0+h,T_1+h]}$  where the  boolean signal $\chi(\vec s , \tau,\phi )$  remains fixed, while the kernel moves accordingly. Essentially, $\tau' \in T$ contributes to $g(t)$ with an additive term of $k_T (\tau'-(t+T_0)) \chi(\vec s , \tau',\phi )$. On the contrary, it contributes to $g(t+h)$ with the additive term $k_T (\tau'-(t+h+T_0)) \chi(\vec s , \tau',\phi )$ which might be not directly comparable with the previous one.
%Good results can be obtained 
If the kernel is a constant function (i.e., $\forall x \in \R,\, k(x)=k_0$), linear ($\forall x,y \in \R,\,k(x+y) = k(x) +  k(y)$), or exponential (i.e., it satisfies the  semigroup property  $\forall x,y\in \R,\,k(x+y) = k(x) \cdot  k(y)$), this can be efficiently done: 
%In this cases, in fact, the evaluation of $g(t)-p$ can be performed efficiently, as shown below for the constant, exponential and linear kernel defined in Table \ref{tab:kernel}. \newline
\begin{itemize}
\item \textbf{Constant}: \small{$
 g(t+h)-p = g(t)-p  + I_{k_T} {({t+T_1},{t+T_1+h})}-$}  \small{$I_{k_T} {({t+T_0}, {t+T_0+h})}$}.
\item \textbf{Exponential}: \small{$
 g(t+h)-p = g(t)-p  + I_{k_T} {({t+T_1},{t+T_1+h})}- I_{k_T} {({t+T_0},{t+T_0+h})} + p(1-e^{-\alpha h})$}.
\end{itemize}
where
$I_{k_T} (a,a+h) = \int_{a}^{a+h}K_T(\tau - a)\chi(\vec s , \tau,\phi ) d\tau$.

% \noindent \textbf{Constant kernel}
% $$
%  g(t+h)-p = g(t)-p  + I_{k_T} {({t+T_1},{t+T_1+h})}- I_{k_T} {({t+T_0},{t+T_0+h})}.
% $$

% \noindent \textbf{Exponential kernel} 
% \begin{eqnarray*}
%  g(t+h)-p  &=& e^{-\alpha h}(g(t)-p  + I_{k_T} {({t+T_1},{t+T_1+h})}- I_{k_T}{({t+T_0},{t+T_0+h})}\\
%  &+&p(1-e^{-\alpha h}).
% \end{eqnarray*}

% %\noindent \textbf{Linear kernel}
% %\begin{eqnarray*}
% % g(t+h)-p  &=& g(t)-p  + I_{k_T} {({t+T_1},{t+T_1+h})}- I_{k_T} {({t+T_0},{t+T_0+h})}\\
% % &-& \frac{mh}{(m/2)(T_1-T_0) + q} \gamma(t+h).
% %\end{eqnarray*}
% %where $\gamma$  is the convolution between the boolean signal and the constant kernel and
% where
% $$
% I_{k_T} (a,a+h) = \int_{a}^{a+h}K_T(\tau - a)\chi(\vec s , \tau,\phi ) d\tau.
% $$
These relationships can be easily exploited to obtain an algorithm that computes the values of $g(t)-p$. The computation can be optimised by suitably tracking the times in which the signal $\chi(\vec s, \tau,\phi )$ switches values. The algorithm is fully reported in Appendix \ref{app:monitoring}. 


If the kernel $k_T$ is not one of the previous types, we need to resort to a more general and expensive method, yet having the same asymptotic complexity, as we can still reuse previously computed values of $g(t)$, provided we decompose the input signal. 
To see how to proceed in the general case, assume the signal $\chi(\vec s, \tau,\phi )$ to be \emph{unitary}, namely that it is true in a single interval of time, say from time $u_0$ to time $u_1$, and false elsewhere. 
In this case, it easily follows that the convolution with the kernel will be non-zero only if the interval $[u_0,u_1]$ intersects the convolution window $t+T$. Inspecting Figure \ref{fig:monitor}, we can see that sliding the convolution window forward of a small time $h$ corresponds to sliding the positive interval of the signal $[u_0,u_1]$ of $h$ time units backwards. In case 
$[u_0,u_1]$ is fully contained into $t+T$, by making $h$ infinitesimal and invoking the fundamental theorem of calculus, we can compute the derivative of $g(t)$ with respect to time as $\frac{d}{dt}g(t) = k_T(u_0 - (t+T_0)) - k_T(u_1 - (t+T_0))$. By taking care of cases in which the overlap is only partial, we can derive a general formula for the derivative:
\begin{equation}
\label{eq:generalODEpositiveInterval}
\frac{d}{dt}g(t) = k_T(u_0 - (t+T_0))I\{u_0\in t+T\} - k_T(u_1 - (t+T_0))I\{u_1\in t+T\},
\end{equation}
where $I$ is the indicator function. This equation can be seen as a differential equation that can be integrated with respect to time by standard ODE solvers (taking care of discontinuities e.g. by stopping and restarting the integration at boundary times when the signal changes truth value), returning the value of the convolution for each time $t$. The initial value is $g(0)$, that has to be computed integrating explicitly the kernel (or setting it to zero if $u_0\geq T_1$).
If the signal $\chi(\vec s , \tau,\phi )$ is not unitary, we have to add  a term like the right hand side of \refeq{eq:generalODEpositiveInterval} in the ODE of $g(t)$ for each unitary component (positive interval) in the signal. 
%to split it into the unitary components and integrate one ODE for each component, adding them up to obtain the proper value of the convolution.
We can also use a root finding algorithm integrated in the ODE solver to detect when the property will be true or false, i.e. when $g(t)$ will be above or below the threshold $p$.
This offline algorithm can be turned into an online procedure by dynamically adding terms in the ODE for $g(t)$. 


% that can be optimized by integrating only the ODEs of those unitary signals that can contribute to $g(t)$ at each $t$, i.e. whose positive interval intersects the convolution window positioned in $t$. Dynamically adding and removing variables in the ODE integration can be a strategy to obtain an online monitor. 

In order to monitor the quantitative semantics, in this paper we used a simple approach: we run the boolean monitor for different values of $r$ in a grid, and then identify the correct value of $r$ by intensifying the search when $g(t)-p$ changes sign. A more efficient procedure for quantitative monitoring is in the top list of future works.  \todo{paragrafo poco chiaro}

\vspace{-5mm}
\begin{figure}
\begin{center}
\includegraphics[width=0.8\textwidth]{img/algo2}
\end{center}
\caption{Sketch of the general monitoring algorithm. The green arrows represents $[u_0,u_1]$ in the constitutional window at time $t$, the red arrows instead represents the same interval at time $t+h$ (backwards translation).}
\label{fig:monitor}
\end{figure}




% Let us denote with $\mathcal{M}_{\phi}$ the monitoring algorithm (monitors) of $\phi$. It produces as output tuple $\{(t_i,b_i) \}_{i\ge 0}$ which are stored directly into two buffer queues $qT_\phi$ and $qB_\phi$. The first queue contains the times $\{t_i\}_{i\ge 0}$ and the second queue contains the boolean values $\{b_i\}_{i\ge 0}$ such that if $b_i = 1$ than $ \forall t \in [t_i,t_{i+1}),\,(t, \vec s) \models \phi$, otherwise if $b_i = 0$  than $ \forall t \in [t_i,t_{i+1}),\,(t, \vec s) \not \models \phi$. This queues are than shared to other monitors which need the values stored in, for example the algorithm $\mathcal{M}_{\phi_1 \wedge \phi_2 }$ can access to $qT_{\phi_1}$,$qB_{\phi_1}$,$qT_{\phi_2}$,$qB_{\phi_2}$.  
% In \ref{alg:monitoring} we shows the monitor of formulas with temporal operator $\langle k_{[T_0,T_1]}, p \rangle \phi$. The monitors of other kind of formulas are pretty straightforward.

%  Let us consider the monitor $ \mathcal{M}_{\langle k_{[T_0,T_1]}, p \rangle \phi}$ (Algorithm \ref{alg:monitoring}). It is composed by three phases. The \emph{initialization phase} (line $2-9$) where the algorithm  waits until the first reaction occurs inside the convolution windows (i.e $[t+T_0,t+T_1]$). The \emph{storing phase} (line $10 - 16$) where the algorithm stores information until a reaction outside the convolution windows occurs. The \emph{evaluation phase} (line $17 - 33$) where the algorithm is ready to calculate the boolean semantics in $t$ and for the next reactions until the final monitoring time ($t_{end}$) is met.

% In the initialization phase, after the variables initialization, a while loop (line $5 - 8$) is performed. Its purpose is to initialize the $b_i$ variable to the values of the boolean semantics of $\phi$ evaluated in $t_i = t+K.T_0$. 

% In the storing phase, which starts in line $10$, the monitor moves the elements from the queue $qT_{\phi}$,$qB_{\phi}$ to the internal queues \texttt{time} and \texttt{space}, respectively, until the time obtained by $qT_{\phi}$ is outside of the convolution windows (see the while condition at line 10). During the storing phase the threshold variables \texttt{th} is updated (line $14$) and the variables $\mathtt{b_f}$ points to boolean semantics of $\phi$ evaluated in $\mathtt{t_f}= \mathtt{t}+\mathtt{K.T_1}$.  The variable \texttt{th} is related to the monitoring of $ \langle k_{[T_0,T_1]}, p \rangle \phi $. A positive values means that  $ \langle k_{[T_0,T_1]}, p \rangle \phi $ is satisfied. On the contrary, a negative values means  $ \langle k_{[T_0,T_1]}, p \rangle \phi $ is not satisfied. For this reason,  the simple idea of this online monitoring algorithm consists in monitoring when $\mathtt{th}$ changes sign.At the end of the storing phase we are able to produce the output of the monitor in time \texttt{t} and moving the convolution windows to the right so to evaluate the boolean semantics for $t> \texttt{t}$. 

% When we enter into the evaluating phase (line $20$), we have two internal queue  \texttt{time} and \texttt{space} which store all the necessary data to update the threshold $\mathtt{th}$ and consequently to calculate the boolean semantics of the target formula. There are two pointer $\mathtt{t_i}$ which points to a time before the first elements stored in  $\texttt{time}$ and $\mathtt{t_f}$ which points to the last element stored in $\texttt{time}$. The interval $[\mathtt{t_i},\mathtt{t_f}]$ represents the convolution windows which is necessary to apply in order to achieve the boolean semantics of the formula $\phi$ in $\mathtt{t}$. As soon as a new tuple arrives $(t_{new},b_{new})$ we are able to move the convolution windows from  $[\mathtt{t_i},\mathtt{t_f}]$ to $[\mathtt{t_i}+h,\mathtt{t_f}+h]$ where $h=t_{new} - \mathtt{t_f}$. It means that the algorithm is able to monitor the boolean semantics from $\mathtt{t}$  to $\mathtt{t_i}+h$. The idea is to check during this translation to the right if and the exact moment the variables \texttt{th} changes sign. 
% This entire procedure is achieved by the while loop (line $21 - 36$). 
% This is achieved by the method \textsc{solve} in line 24 and 30. As we noticed the translation is not performed in a row but there are two cases [\ldots]. The monitoring algorithm is than performed until the the specified time ($t_{end}$) is reached (see the while-loop condition at line 20)

% %
% % we have stored in $(t_{i},b_{i})$ the first output of the monitoring $\mathcal{M}_\phi$ which belongs to the convolution windows.  
% %
% %      
% %
% %
% %The main procedure in the \textsc{monitor} (line 1) which takes as input the time ($t$) when we want to start the monitoring, the kernel ($K$) which is an object with two fields $K.T_0,K.T_1$ describing the kernel window and has a method ($K.int(a,b)$) which calculates the integral of the kernel between $a$ and $b$. The input ($p$) is the percentage of the formula and $qT$ and $qB$ are two FIFO queues. As soon as a new reaction occurs its time ($t_{new}$) and $b_{new} = \chi(\phi,\vec s , \tau )$ are momentarily stored in the buffers queue $qT$ and $bT$, respectively. For simplicity we define a set of global variables (line 2) which are shared among all the procedures. There are two queues \texttt{signal} and \texttt{time}. Their elements are accessible by an integer index i.e \texttt{time}[index], notice that \texttt{time}[-1] means the last element on the queue, or by the usual pop() method which returns the first element and erase it from the queue. After the initialization of the global variables the \textsc{monitor} procedure call the \textsc{init} procedure on the data collected by the first reaction after the beginning of the monitoring (line 5) (i.e, \texttt{qT}.pop() and \texttt{qB}.pop()). If these queues are empty,  the algorithm wait until a new element arrives.
% %The \textsc{init} procedure goal is to wait the necessary time to perform the monitoring in the initial time $t$ and prosecuting to the following times.In the if-else code (line 9 -14) we wait until the first reaction occurs inside the monitoring window. We save the boolean signal in the queue \texttt{signal}[0] and the starting time  of the window in the queue \texttt{time} (line 13). In the next if-else statement (line 15-23) we wait until the first reaction after the windows occurs (i.e., $t_{new}\ge \mathtt{t}+\mathtt{K.T_1}$),  in the mean time the algorithm perform the convolution integration step by step (line 16) and store the value in the variables \texttt{th}. The sign of this variable represents the boolean semantics we are going to calculate. \textsc{init} procedure terminates in line 22 where the \textsc{waiting} procedure is called. In the waiting procedure we are ready to move the convolution windows and monitor the values of the semantics for higher values than \texttt{t}. From the previous procedure we have two pointer \texttt{tf}= \texttt{time}[-1] and \texttt{time}[0] which points to the beginning and to the end of the queue \texttt{time}. When a new reaction occurs ($t_{new}$)the algorithm stores its data and move this two pointer accordingly on the time queue, in order to discard all the time reactions which are no more included in the windows. We are simply translating the windows to the right of $t_{new} - \mathtt{tf}$ unit of time.

% \begin{algorithm}[ht]
% \caption{}\label{alg:monitoring}
% \begin{algorithmic}[1]
% \Procedure{monitor($t,kernel,p$)}{}
% \State $\mathtt{t} \gets t,\,\mathtt{K} \gets kernel,\,\mathtt{t_f} \gets t,\,\mathtt{th} \gets -p$
% \State $\mathtt{signal} \gets [],\,\mathtt{time} \gets [],\,\mathtt{qT} \gets qT,\,\mathtt{qB} \gets qB$
% \State $ t_{new} \gets \mathtt{t}  $
% \While{ ($t_{new}\le \mathtt{t}+\mathtt{K.T_0}$)}
% \State $b_{i} \gets \text{\texttt{qB}.pop()}$
% \State $ t_{new} \gets \text{\texttt{qT}.pop()}  $
% \EndWhile
% \State $\mathtt{t_i} \gets \mathtt{t}+\mathtt{K.T_0}$
% \State $\mathtt{t_{app}} \gets \mathtt{t_i}$
% %\State $b_{new} \gets b_{new}$
% %\State \texttt{time}.push($\mathtt{t}+\mathtt{K.T_0}$)
% %\State \texttt{signal}.push($b_{new}$)
% %\State $b_{new} \gets \texttt{qB}.pop()$
% \While{ ($t_{new}\le \mathtt{t}+\mathtt{K.T_1}$)}
% \State \texttt{time}.push($t_{new}$)
% \State \texttt{signal}.push($b_{new}$)
% \State $\texttt{th} \gets \texttt{th} + \mathtt{b_f} \cdot \text{\texttt{K}.integrate}(\mathtt{t_{app}} - \mathtt{t_i},t_{new}-\mathtt{t_i} )$
% \State $\mathtt{t_{app}} \gets t_{new}$
% \State $\mathtt{b_f}\gets b_{new}$
% \State $ (t_{new},b_{new}) \gets (\text{\texttt{qT}.pop()}, \text{\texttt{qB}.pop()}$)
% \EndWhile
% \State $\mathtt{t_f}\gets \mathtt{t}+\mathtt{K.T_1} $
% \While{$\mathtt{t_f} < t_{end}$ }
% \While{ $\mathtt{t_f} < t_{new}$}
% \If{ ($\text{\texttt{time}.peek()}-\mathtt{t_i}\le t_{new} - \mathtt{tf}$)}
% \State $h \gets (\text{\texttt{time}.peek()}-\mathtt{t_i})$
% \State $\texttt{th} \gets \textsc{solve}(\texttt{th},h,\mathtt{b_i},\mathtt{b_f},\mathtt{K})$
% \State $\mathtt{t_i} \gets \text{\texttt{time}.pop()}$
% \State $\mathtt{b_i} \gets \text{\texttt{signal}.pop()}$
% \State $\mathtt{t_f} \gets  \mathtt{t_f} + h $
% \Else
% \State $h \gets t_{new} - \mathtt{tf}$
% \State $\texttt{th} \gets \textsc{solve}(\texttt{th},h,\mathtt{b_i},\mathtt{b_f},\mathtt{K})$
% \State $\mathtt{t_i} \gets \mathtt{t_i}+ h $
% \State $\mathtt{t_f} \gets  t_{new} $
% \State $\mathtt{b_f} \gets  b_{new} $
% \EndIf
% \State $\texttt{t} \gets \texttt{t} + h$
% \EndWhile
% \State $ (t_{new},b_{new}) \gets (\text{\texttt{qT}.pop()}, \text{\texttt{qB}.pop()}$)
% \EndWhile
% \EndProcedure


% \end{algorithmic}
% \end{algorithm}


==> todo.tex <==
% !TEX root =  main.tex
\noindent
\todo{
Principali cose da fare:
\begin{itemize} 
\item logiche meno sensibili al rumore, vedere effettivamente se il review due ha ragione  (\ezio{})
\item implementaz,(algoritmo, nuove prop , mettere codice online)(\simone{})
\end{itemize}
}

